Radiation, entanglement and islands from a boundary local quench

We study the entanglement and the energy density of the radiation emitted after a local quench in a boundary conformal field theory. We use the operator product expansion (OPE) to predict the early- and late-time behavior of the entanglement entropy and we find, under mild assumptions, a universal form for the leading term, which we test on some treatable two-dimensional examples. We also derive a general upper bound on the entanglement, valid along the full time evolution. In two dimensions, the bound is computed analytically, while in higher dimensions it is evaluated at early and late time via the OPE. These CFT predictions are then compared with a doubly-holographic setup where the CFT is interpreted as a reservoir for the radiation produced on an end-of-the-world brane. After finding the gravitational dual of a boundary local quench, we compute the time evolution of the holographic entanglement entropy, whose late-time behavior is in perfect agreement with the CFT predictions. In the brane+bath picture, unitarity of the time evolution is preserved thanks to the formation of an island. The holographic results can be recovered explicitly from the island formula, in the limit where the tension of the brane is close to the maximal value.

==> sections/EarlyLateTime.tex <==
%!TEX root = ../EE_radiation_BCFT.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Light excited states}
\subsection{The Ising model}

which can be computation using Wick's theorem with the two-point
\begin{equation}
	\langle \psi(u_1) \psi(u_2) \rangle = \frac{1}{u_1-u_2}\ .
\end{equation}

$e^{(1-n)\Delta S_n}$ has to be a function of the ratio 
\begin{equation}
	r=\frac{u_2}{u_1}\ ,
\end{equation}
and it also has to be symmetric for the exchange $r\rightarrow\frac{1}{r}$. Indeed if we write $u_2 = r u_1$, we can collect a factor $u_{1}^{1-n}$ from the Jacobian
\begin{equation}
	J= \prod_{i=1}^2 \prod_{j=1}^{n} \left(\frac{\dd u}{\dd w}\right)^{-1/2}_{w=w_{i,j}}  = \frac{1}{n^n} (u_1\, u_2)^{\frac{1-n}{2}}\ ,
\end{equation}
a factor $(u_{1}^{\frac{1}{n}})^{-n}=u_1^{-1}$ from the $2n$-point function in the numerator and $u_1^{n}$ from the normalisation of the fermion operators:
\begin{equation}
	\langle \psi(u_1) \psi(u_2) \rangle^n = \frac{1}{u_1^n\,(1-r)^n}\ .
\end{equation}
Therefore we can set
\begin{equation}
	u_{1} \rightarrow 1 \hspace{0.75cm} \mathrm{and} \hspace{0.75cm} u_{2} \rightarrow r\ .
\end{equation}
This substitution simplifies a lot the computation of the Rényi entropies and the final result can be written in terms of the cross-ratio $\zeta$ in \eqref{eq::crossratio} as
\begin{equation}
	\zeta= \frac{1}{4}\left(2-r-\frac{1}{r}\right)\ .
\end{equation}
\todo{controllare}

We can write an general expression for the $n^{\rm th}$ Rényi entropy as a polynomial of degree $\lfloor\frac{n}{2}\rfloor$ in the cross-ratio:
\begin{equation}
	e^{(1-n)\,S_{n}} = \prod_{k=1}^{\lfloor\frac{n}{2}\rfloor} \left[1-\frac{(n-2k+1)^2}{n^2}\, \zeta\right]\ .
\end{equation}
This expression has been found from analytic computation for $n=2,\ldots ,6$ and checked numerically for higher $n$.

Thus
\begin{equation}
\label{SnFreeF}
	\begin{split}
		S_n &= \frac{1}{1-n}\, \sum_{k=1}^{\lfloor \frac{n}{2} \rfloor} \log\left[ 1 - \frac{(n-2k+1)^2}{n^2}\, \zeta \right] \\
		&= \frac{1}{1-n}\, \sum_{k=1}^{\infty} \frac{1}{k}\left(\frac{4\zeta}{n^{2}}\right)^k \zeta (-2k,\frac{n+1}{2})\ ,
	\end{split}
\end{equation}
where $\zeta (s,q)$ is the {\it Hurwitz zeta} function. \mm{Second line still converges because for integer $i$ the coefficients are decreasing.} \mm{OPE limit seems to work but numerical coefficient to be checked carefully. General formula for the coefficient is $\Delta_\psi \Delta_\sigma/C_D$, and $\Delta_\sigma=c(n^2-1)/(12n^2)$. Factor 2 are moving around and everything to be checked and compared with stress-tensor as external state. This lends support to the fact that the series works as an asymptotic series. (Up to which order?)}

The entanglement entropy is then
\begin{equation}
\label{SEEFreeF}
	\begin{split}
		S_{\rm EE} &= - \sum_{k=1}^{\infty} (4 \zeta)^k \zeta (1-2k)\\ 
		&= \frac{1}{2} \sum_{k=1}^{\infty} \frac{(4\xi)^k}{k} B_{2k} \\
		&= \log \left(\frac{1}{2\sqrt{\xi}}\right) - \psi\left(\frac{1}{2\sqrt{\xi}}\right) - \sqrt{\xi}\ ,
	\end{split}
\end{equation}
where $\zeta(s) = \zeta(s,1)$ is the {\it Riemann zeta} function, $B_n$ are the Bernoulli numbers and $\psi(s)$ is the {\it digamma} function, defined as the logarithmic derivative of the gamma function. \mm{All of this is subject to a leap of faith because the first line in \eqref{SEEFreeF} is asymptotic. Must explain. If late time limit works, this lends support to validity as asymptotic series.}

\begin{figure}[ht]
	\centering
	\includegraphics[width=10cm]{Images/Page-Ising-I+.pdf}
\end{figure}

The Entanglement Entropy for the two different configurations: blue the twist operator on $\mathcal{I}^+$ and orange the twist operator on the time-like curve $x_0=-1$. 

\subsection{The stress-tensor state in a generic CFT}

\begin{equation}
	\langle T(z_1) T(z_2) \rangle = \frac{c}{2 (z_1 - z_2)^4}\ ,
\end{equation}
where $c$ is the {\it central charge}.

The generic $(n+1)$-point correlation function of stress-energy tensor can be found using the recursion relation \cite{Belavin:1984vu}:

\begin{equation}
	\begin{split}
		\langle T(z) T(z_1) \cdots T(z_n) \rangle &= \sum_{i=1}^n \left[ \frac{2}{(z-z_i)^2} + \frac{1}{z-z_i}\partial_{z_i}\right] \langle T(z_1) \cdots T(z_n) \rangle\\
		&\;+\sum_{i=1}^n \frac{c}{2(z-z_i)^4}\, \langle T(z_1) \cdots T(z_{i-1}) T(z_{i+1}) \cdots T(z_n) \rangle
	\end{split}
\end{equation}

\todo{sistemare formule}

\begin{equation}
	\Delta S_{n} =\frac{1}{1-n}\, \log \frac{\langle \sigma(0)\, T^{\otimes n}(u_{1}) T^{\otimes n}(u_{2}) \rangle}{\langle \sigma(0)\rangle\langle T(u_1) T(u_2) \rangle^n}\ ,
\end{equation}

\begin{equation}
	T(u) = \left(\frac{\dd u}{\dd w}\right)^{-2} \left[T^\prime (u) - \frac{c}{12} \{u,w\}\right]\ ,
\end{equation}
where the Schwarzian derivative for the uniformising transformation is
\begin{equation}
	\{u,w\} = \frac{1-n^2}{2\, w^2}
\end{equation}
\todo{il contributo dello Schwarziano tende a zero nel limite $n\to 1$}

\begin{equation}
	\begin{split}
		e^{(1-n)\Delta S_{n}} &= \frac{(u_1 u_2)^{2-2n}}{n^{4n}} \frac{\langle \bigotimes_{i=1}^n T(w_{1,i}) T(w_{2,i}) \rangle}{\langle T(u_1) T(u_2) \rangle^n}\\[.2em]
		&\simeq \frac{(u_1 u_2)^{2-2n}}{n^{4n}} \frac{\prod_{i=1}^n \langle T(w_{1,i}) T(w_{2,i}) \rangle}{\langle T(u_1) T(u_2) \rangle^n}\\[.2em]
		&= \frac{(u_1 u_2)^{2-2n}}{n^{4n}} \left(\frac{u_1-u_2}{u_1^{1/n}-u_2^{1/n}}\right)^{4n} = 1 - \frac{2(n^2-1)}{3n}\zeta+\mathcal{O}(\zeta^2)
	\end{split}
\end{equation}
\todo{se uno prende il limite $c\to \infty$ prima, allora questo non e' il contributo leading}

\begin{equation}
	\begin{split}
		\Delta S_n = \frac{2 (n+1)}{3n} \zeta +\mathcal{O}(\zeta^2)\ ,\\
		\Delta S_{EE} = \frac{4}{3} \zeta +\mathcal{O}(\xi^2)\ ,
	\end{split}
\end{equation}

\begin{figure}[ht]
	\begin{multicols}{3}
		\includegraphics[width=\linewidth]{Images/StressTensor05I+.pdf}
		\includegraphics[width=\linewidth]{Images/StressTensor084I+.pdf}
		\includegraphics[width=\linewidth]{Images/StressTensor1I+.pdf}
	\end{multicols}
	\begin{multicols}{3}
		\includegraphics[width=\linewidth]{Images/StressTensor10I+.pdf}
		\includegraphics[width=\linewidth]{Images/StressTensor20I+.pdf}
		\includegraphics[width=\linewidth]{Images/StressTensor10000I+.pdf}
	\end{multicols}
\end{figure}

\begin{equation}
	\begin{split}
		\mathrm{Tr} \rho K^{0} &=- \int_{0}^{1} y \left(\frac{\langle T(z_1) T(z_2) T(y)\rangle}{\langle T(z_1) T(z_2) \rangle} + \frac{\langle \overline{T}(\bar{z}_1) \overline{T}(\bar{z}_2) \overline{T}(\bar{y})\rangle }{\langle \overline{T}(\bar{z}_1) \overline{T}(\bar{z}_2)\rangle}\right) \dd y\\[.2em]
		&=2\left(2 + \frac{z_1+z_2}{z_1-z_2} \log \frac{z_2}{z_1} \right) \simeq \frac{4}{3} \xi +\mathcal{O}(\xi^2) \ ,
	\end{split}
\end{equation}
which is invariant as expected under $z_1 \leftrightarrow z_2$.

==> sections/Solutions.tex <==
%!TEX root = ../EE_radiation_BCFT.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{End-of-the-World Brane solutions in \texorpdfstring{AdS$_3$}{AdS3}}

\begin{equation}
    \dd s^2_{\rm thermal} \left(\frac{z_H}{z_0}\right)= R^2 \left(\frac{\dd \tau^2}{z^2} + \frac{h_0(z)}{z^2} \dd x^2 + \frac{\dd z^2}{h_0(z) z^2}\right)\ ,
\end{equation}
and
\begin{equation}
    \dd s^2_{\rm BTZ} \left(\frac{z_H}{z_0}\right)= R^2 \left(\frac{\dd x^2}{z^2} + \frac{h_H(z)}{z^2} \dd \tau^2 + \frac{\dd z^2}{h_H(z) z^2}\right)\ ,
\end{equation}
with $\tau \sim \tau + 2\pi z_H$, $x\sim x + 2\pi z_0$, $h_0(z) = 1- \left(\frac{z}{z_0}\right)^2$ and $h_H(z) = 1- \left(\frac{z}{z_H}\right)^2$.

\begin{equation}
    \dd s^2_{\rm BTZ} \left(\frac{z_0}{z_H}\right) \underset{\tau \leftrightarrow x}{=} \dd s^2_{\rm thermal} \left(\frac{z_H}{z_0}\right)
\end{equation}

The brane cuts off one identification:
